Unifying and Strengthening Hardness for Dynamic Problems via the Online Matrix-Vector Multiplication Conjecture

Consider the following Online Boolean Matrix-Vector Multiplication problem: We are given an $n\times n$ matrix $M$ and will receive $n$ column-vectors of size $n$, denoted by $v_1,\ldots,v_n$, one by one. After seeing each vector $v_i$, we have to output the product $Mv_i$ before we can see the next vector. A naive algorithm can solve this problem using $O(n^3)$ time in total, and its running time can be slightly improved to $O(n^3/\log^2 n)$ [Williams SODA'07]. We show that a conjecture that there is no truly subcubic ($O(n^{3-\epsilon})$) time algorithm for this problem can be used to exhibit the underlying polynomial time hardness shared by many dynamic problems. For a number of problems, such as subgraph connectivity, Pagh's problem, $d$-failure connectivity, decremental single-source shortest paths, and decremental transitive closure, this conjecture implies tight hardness results. Thus, proving or disproving this conjecture will be very interesting as it will either imply several tight unconditional lower bounds or break through a common barrier that blocks progress with these problems. This conjecture might also be considered as strong evidence against any further improvement for these problems since refuting it will imply a major breakthrough for combinatorial Boolean matrix multiplication and other long-standing problems if the term "combinatorial algorithms" is interpreted as "non-Strassen-like algorithms" [Ballard et al. SPAA'11]. The conjecture also leads to hardness results for problems that were previously based on diverse problems and conjectures, such as 3SUM, combinatorial Boolean matrix multiplication, triangle detection, and multiphase, thus providing a uniform way to prove polynomial hardness results for dynamic algorithms; some of the new proofs are also simpler or even become trivial. The conjecture also leads to stronger and new, non-trivial, hardness results.

==> warmup.tex <==
\section{Showcases}\label{sec:warmup}

In this section we present two simple reductions as showcases for how to reduce from problems in the previous section. In \Cref{sec:warmup1}, we show a reduction from the \ouMv problem. A reduction of this type usually implies that a dynamic problem requires a high query time. In \Cref{sec:warmup2}, we show a reduction from the hinted \ouMv problem. This kind of reductions usually imply a trade-off between query and update time.\danupon{IMPORTANT: The statements below should make this point clear.}\thatchaphol{NEED CHANGE because there is no $\houMv{\delta}$ now.}

\subsection{Incremental $s$-$t$ Shortest Path (st-SP).}\label{sec:warmup1}
Based on the hardness of $\ouMv$ we get a lower bound of $ \oo (n^3) $ for the incremental $s$-$t$ shortest path problem when $m=\Theta(n^{2})$.
Note that there is a matching upper bound of total update time $O(m n)$ due to \cite{EvenS81}.
This raises the question whether one can also obtain lower bounds for sparser graphs.
In \Cref{sec:full:partially hardness}, we will show that this is possible by extending our technique.



\begin{lemma}\label{lem:reduction_incremental_st_SP}
Given an incremental algorithm $\cA$ for st-SP, one can solve $\ouMv$ with parameters $n_1,n_2,n_3$ by running $\cA$ in an initially empty graph with 
$\Theta(n_{1}+n_{2}+n_{3})$ vertices,
and using $O(n_{1}n_{2}+n_{1}n_{3}+n_{2}n_{3})$ edge insertions, $n_3$ queries.
\end{lemma}
\begin{proof}
Given $M$, we construct the bipartite graph $G_{M}=((L,R),E)$ where
$L=\{l_{1},\dots,l_{n_{1}}\}$, $R=\{r_{1},\dots,r_{n_{2}}\}$, and
$E=\{(r_{j},l_{i})\mid M_{ij}=1\}$.
%
We construct two paths $P$ and $Q$ with $n_{3}$ vertices each.
Let $P=(p_{n_{3}},p_{n_{3}-1},\dots,p_{1})$ where $p_{n_{3}}=s$,
and $Q=(q_{1},q_{2},\dots,q_{n_{3}})$ where $q_{n_{3}}=s'$. 
%
Once $u^{t}$ and $v^{t}$ come, we connect $p_{t}$ to $l_{i}$ iff
$u_{i}^{t}=1$, for all $1 \le i \le n_1$, 
and connect $q_{t}$ to $r_{j}$ iff $v_{j}^{t}=1$, for all $1 \le j \le n_2$.
We have that if $(u^{t})^{\top}Mv^{t}=1$, then $d(s,s')=2(n_{3}-t)+1$,
otherwise $d(s,s')\ge2(n_{3}-t)+2$. \end{proof}
\begin{corollary}
\Cref{oMv hard} implies that there is no incremental st-SP algorithm processing a sequence of $ \Theta (n^2) $ insertions and $ n $ queries with
total update time $\oo(n^{3})$ and time $\oo(n^{2})$ per query.\end{corollary}
\begin{proof}
Suppose there is such an algorithm. By \Cref{lem:reduction_incremental_st_SP}, we can solve
$\ouMv$ when $n_{1}=n_{2}=n_{3}=n$ in time $\oo(n^{3})$. 
\end{proof}
This implies that the amortized time per insertion cannot be $ \oo(n) $ when the final graph is dense.



\subsection{Single-source subgraph connectivity (ss-SubConn).}\label{sec:warmup2}
The following reduction to ss-SubConn uses similar ideas as the one to st-SP.

\begin{lemma}
	\label{lem:ss-subconn reduc showcase}Given a partially dynamic algorithm $\cA$ for ss-SubConn, after polynomial preprocessing time, 
	one can solve $\uMv$ with parameters $m^\delta,m^{1-\delta}$ by running $\cA$ on a graph with $\Theta(m^{1-\delta}+m^{\delta})$ nodes and $O(m)$ edges,
	then using $O(m^{1-\delta})$ insertions (or $O(m^{1-\delta})$ deletions) and $O(m^{\delta})$	queries.\end{lemma}
\begin{proof}
	We show only the decremental case because the incremental case is
	symmetric. Given $M$, we construct the bipartite
	graph $G_{M}=((L,R),E)$ where $L = {l_1,\dots,l_{m^\delta}}$ and $R = {r_1,\dots,r_{m^{1-\delta}}}$, and 
	$E=\{(r_{j},l_{i})\mid M_{ij}=1\}$, with an additional vertex $s$ and edges $(r_{j},s)$
	for all $j\le m^{1-\delta}$. Thus, the total number of edges is $m+m^{1-\delta}$.
	%
	In the beginning, every node is turned on.
	%
	Once $u$ and $v$ come, we turn off $r_{j}$ iff $v_{j}=0$. If $u^{\top}Mv=1$,
	then $s$ is connected to $l_{i}$ for some $i$ where $u_{i}=1$.
	Otherwise, $s$ is not connected to $l_{i}$ for all $i$ where $u_{i}=1$.
	In total, we need to do $O(m^{1-\delta})$ updates and $O(m^{\delta})$
	queries.
\end{proof}

\begin{corr}
	\label{cor:ss-subconn hard showcase}
	For any constant $\delta\in (0,1)$, \Cref{oMv hard} implies that 
	there is no algorithm for partially dynamic ss-SubConn on a graph with $n$ nodes and 
	$m = O( \min(n^{1/\delta} , n^{1/(1-\delta)} )$ edges
	with preprocessing time $p(m)=poly(m)$, worst case update time $ u(m) =\oo(m^{\delta})$, 
	and query time $ q(m) =\oo(m^{1-\delta})$.
	This is also true for the amortized update time in fully dynamic algorithms.s
\end{corr}

\begin{proof}
	Let $\cA$ be such a partially dynamic algorithm. Note that the number of edges in the graph in the reduction in \Cref{lem:ss-subconn reduc showcase} is $m = O( \min(n^{1/\delta} , n^{1/(1-\delta)} )$.
	So, by \Cref{lem:ss-subconn reduc showcase}, after polynomial time preprocessing, 
	one can solve $\uMv$ with parameters $m^\delta,m^{1-\delta}$ in time $O(m^{1-\delta}u(m) + m^{\delta}q(m)) = \oo(m)$. 
	This contradicts \Cref{oMv hard} by \Cref{uMv hard}.
	
	Next, suppose that $\cA$ is fully dynamic and guarantees only amortized bound. That is, if there is at most $m$ edges ever appeared in the graph, then after a sequence of $t \ge m$ updates, the total update time is $O(t\cdot u(m))$.
	So, by \Cref{lem:ss-subconn reduc showcase} and by ``undoing'' the operations when the new vector pair comes, as $\cA$ is fully dynamic, one can solve $\ouMv$ with parameters $m^\delta,m^{1-\delta},n_3$ in time $\oo(mn_3)$ when $n_3 = m$. This contradicts \Cref{oMv hard} by \Cref{ouMv hard}.
\end{proof}

